Enabling Acoustic Audience Feedback in Large Virtual Events

The COVID-19 pandemic shifted many events in our daily lives into the virtual domain. While virtual conference systems provide an alternative to physical meetings, larger events require a muted audience to avoid an accumulation of background noise and distorted audio. However, performing artists strongly rely on the feedback of their audience. We propose a concept for a virtual audience framework which supports all participants with the ambience of a real audience. Audience feedback is collected locally, allowing users to express enthusiasm or discontent by selecting means such as clapping, whistling, booing, and laughter. This feedback is sent as abstract information to a virtual audience server. We broadcast the combined virtual audience feedback information to all participants, which can be synthesized as a single acoustic feedback by the client. The synthesis can be done by turning the collective audience feedback into a prompt that is fed to state-of-the-art models such as AudioGen. This way, each user hears a single acoustic feedback sound of the entire virtual event, without requiring to unmute or risk hearing distorted, unsynchronized feedback.

==> drawings/jitsi.tex <==
\begin{tikzpicture}
 
    \node (image) at (0,0) {
        \includegraphics[width=\textwidth, trim=8cm 2.5cm 8cm 4cm, clip]{images/jitsi_visualization.pdf}
    };
    \node[text=white] at (7,-3){Image: \url{freepick.com}};
 
\end{tikzpicture}
